Reliable MIMO Optical Wireless Communications Through Super-Rectangular Cover

In this paper, we consider an intensity modulated direct detection MIMO optical wireless communication (OWC) system. For such a system, a novel super-rectangular cover theory is developed to characterize both the unique identifiability and full reliability. This theory states that a transmitted matrix signal can be uniquely identified if and only if the cover order is equal to the transmitter aperture number, i.e., full cover. In addition, we prove that full reliability is guaranteed for space-time block coded MIMO-OWC over commonly used log-normal fading channels with an ML detector if and only if the STBC enables full cover. In addition, the diversity gain can be geometrically interpreted as the cover order of the super-rectangle, which should be maximized, and the volume of this super-rectangle, as the diversity loss, should be minimized. Using this established error performance criterion, the optimal linear STBC for block fading channels is proved to be spatial repetition code with an optimal power allocation. The design of the optimal non-linear STBC is shown to be equivalent to constructing the optimal multi-dimensional constellation. Specifically, a multi-dimensional constellation from Diophantine equations is proposed and then, shown to be more energy-efficient than the commonly used nonnegative pulse amplitude modulation constellation.

==> TNDs_IEEEtran_v16_mods.tex <==
%%%
%%% Redefine maketitle so that abstract and keywords and edics
%%% appear on the first page in draft mode
%%%

\makeatletter

\def\maketitle{\par%
  \begingroup%
  \normalfont%
  \def\thefootnote{}%  the \thanks{} mark type is empty
  \def\footnotemark{}% and kill space from \thanks within author
  \footnotesize%       equal spacing between thanks lines
  \footnotesep 0.7\baselineskip%see global setting of \footnotesep for more info
  \normalsize%
  \if@twocolumn%
     \if@technote%
        \newpage\global\@topnum\z@ \@maketitle\@IEEEstatictitlevskip\@IEEEaftertitletext%
     \else\twocolumn[\@maketitle\@IEEEdynamictitlevspace\@IEEEaftertitletext]\fi%
  \else\newpage\global\@topnum\z@ \@maketitle\@IEEEstatictitlevskip\@IEEEaftertitletext%
  \fi%
  \if@IEEEusingpubid%
   \thispagestyle{pubidtitlepagestyle}\@thanks%
   \enlargethispage{-\@pubidpullup}%
  \else%
   \thispagestyle{titlepagestyle}\@thanks%
  \fi%
  \endgroup%
  \setcounter{footnote}{0}\let\maketitle\relax\let\@maketitle\relax%
  \gdef\@thanks{}\gdef\@author{}\gdef\@title{}%
  \let\thanks\relax%
%TND 16 Aug 02: Commented out line below to get desired effect
  %\if@draftclsmode\vfil\mbox{}\newpage\fi%
}

% Define edics environment

\def\edics{\normalfont%
    \if@twocolumn%
    \else%
      \begin{center}\@IEEEabskeysecsize\bfseries EDICS\end{center}\quotation\@IEEEabskeysecsize%
    \fi\@IEEEgobbleleadPARNLSP}
\def\endedics{\relax\if@technote\vspace{1.34ex}\else\vspace{0.67ex}\fi%
    \par\if@twocolumn\else\endquotation\fi%
    \if@draftclsmode \mbox{}\vfil\fi
    \normalsize\normalfont}


%%%% Set up paper status command in draftcls mode

% set up the running headings, this complex because of all the different
% modes IEEEtran supports
\if@twoside
 \if@technote
   \def\ps@headings{%
       \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
       \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
       \if@draftclsmode
            \def\@oddfoot{\scriptsize\@date\hfil \paperstatus}
            \def\@evenfoot{\scriptsize \paperstatus\hfil\@date}
       \else
            \def\@oddfoot{}\def\@evenfoot{}
       \fi}
 \else % not a technote
   \def\ps@headings{%
       \if@confmode
        \def\@oddhead{}
        \def\@evenhead{}
       \else
        \def\@oddhead{\hbox{}\scriptsize\rightmark \hfil \thepage}
        \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
       \fi
       \if@draftclsmode
            \def\@oddhead{\hbox{}\scriptsize\rightmark \hfil \thepage}
            \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
            \def\@oddfoot{\scriptsize\@date\hfil \paperstatus}
            \def\@evenfoot{\scriptsize \paperstatus\hfil\@date}
       \else
            \def\@oddfoot{}\def\@evenfoot{}
       \fi}
 \fi
\else % single side
\def\ps@headings{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{}
    \fi
    \if@draftclsmode
          \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
          \def\@evenhead{}
          \def\@oddfoot{\scriptsize \@date \hfil \paperstatus}
    \else
         \def\@oddfoot{}
    \fi
    \def\@evenfoot{}}
\fi

% title page style
\def\ps@titlepagestyle{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
    \fi
    \if@draftclsmode
         \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
         \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
         \def\@oddfoot{\scriptsize \@date\hfil \paperstatus}
         \def\@evenfoot{\scriptsize \paperstatus\hfil \@date}
    \else
         \def\@oddfoot{}\def\@evenfoot{}
    \fi}

% pagestyle for pages that have a publisher's ID
% we bring the footer ID text up into the last line of the
% main text
% publisher's ID will not be printed when in DRAFT mode.
\def\ps@pubidtitlepagestyle{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
    \fi
    \if@draftclsmode
         \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
         \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
         \def\@oddfoot{\scriptsize \@date\hfil \paperstatus}
         \def\@evenfoot{\scriptsize \paperstatus \hfil \@date}
    \else
         \footskip 0pt
         \def\@oddfoot{\hss\normalfont\footnotesize\raisebox{1.5ex}[1.5ex]{\@pubid}\hss}
         \def\@evenfoot{\hss\normalfont\footnotesize\raisebox{1.5ex}[1.5ex]{\@pubid}\hss}
    \fi}

\ps@headings
\makeatother

